A note on composition operators on model spaces

Motivated by the study of composition operators on model spaces launched by Mashreghi and Shabankha we consider the following problem: for a given inner function $\phi\not\in\mathsf{Aut}(\mathbb D)$, find a non-constant inner function $\Psi$ satisfying the functional equation $\Psi\circ\phi=\tau\Psi$, where $\tau$ is a unimodular constant. We prove that this problem has a solution if and only if $\phi$ is of positive hyperbolic step. More precisely, if this condition holds, we show that there is an infinite Blaschke product $B$ satisfying the equation for $\tau=1$. If in addition, $\phi$ is parabolic, we prove that the problem has a solution $\Psi$ for $any$ unimodular $\tau$. Finally, we show that if $\phi$ is of zero hyperbolic step, then no non-constant Bloch function $f$ and no unimodular constant $\tau$ satisfy $f\circ\phi=\tau f$.

==> def_latex.tex <==
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{euscript}
%\usepackage[dvips]{graphics}
%\usepackage{epsf}
%\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%\let\script=\EuScript
%\let\cal=\mathcal      

\def\mcc{M\raise.5ex\hbox{c}C}
\def\mccarthy{M\raise.5ex\hbox{c}Carthy}
\def\Hu{\H}
\def\sz{Szeg\Hu{o} } 
\def\szs{Szeg\Hu{o}'s } 
\newcommand{\df}[1] {{\bf #1}}


\def\eg{{\it e.g. }}
\def\ie{{\it i.e. }}

%Hilbert spaces
\def\atm{{\A}^2(\mu)}
\def\atn{{\A}^2(\nu)}
\def\htm{H^2(\mu)}
\def\ptm{P^2(\mu)}
\def\ltm{L^2(\mu)}
\def\h{{\cal H}}
\def\hk{{\cal H}_k}
\def\hs{{\cal H}_s}
\def\K{{\cal K}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\HH{{\cal H}} 
\def\LL{{\cal L}}
\def\kz{{\cal K}_0}
\def\ko{{\cal K}_1}
\def\lz{{\cal L}_0}
\def\lo{{\cal L}_1}

%Banach spaces
\def\limu{L^\infty(\mu)}
\def\hi{H^\infty}
\def\hd{H^\infty(\D)}
\def\hid{H^\infty(\D)}
\def\hb{H^\infty(\D^2)}
\def\m{Mult}

%modified Greek letters
\def\Ga{\Gamma}
\def\ga{\gamma}
\def\De{\Delta}
\def\La{\Lambda}
\def\bla{{\overline{\Lambda}}}
\def\Om{\Omega}
\def\bom{\overline{\Omega}}
\def\a{\alpha}
\def\l{\lambda}
\def\z{\zeta}
\def\li{\lambda_i}
\def\ki{k_{\lambda_i}}
\def\ksi{k^S_{\lambda_i}}
\def\ksj{k^S_{\lambda_j}}
\def\ksn{k^S_{\lambda_{N+1}}}
\def\th{\theta}
\def\ei{e^{i\theta}}
\def\vare{\varepsilon}

%abbreviations
%\let\ii=\i
\let\i=\infty
\def\v{\vert}
\def\V{\Vert}
\def\la{\langle}
\def\ra{\rangle}
\def\={\ = \ }    
\def\ot{\otimes}

%boldface
\def\MM{{\mathbf M}}
\def\Sl{{\mathbf S}_\La}
\def\TT{{\mathbf T}}
\def\WW{{\mathbf W}}

%other
\def\A{{\cal A}}
\def\BB{{\cal B}}
\def\CC{{\cal C}}
\def\F{{\cal F}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\PP{{\cal P}}
\def\E{E_\l}
\def\Eb{E_{\bar \l}}
\def\Ee{{\cal E}_{\l}}
\def\Lc{{\cy7 L}}
\def\zz{{\cy7 Z}}
\def\ba{{\cy7 B}}
\def\dkw{{\rm dim}(k,w)}
\def\DD{D_\delta(k,w)}
\def\ws{{w^\sharp}}
\def\kp{{k^\prime}}
\def\kpp{{k^{\prime \prime}}}
\def\ellp{{\ell^{\prime}}}
\def\ellpi{{\ell_i^{\prime}}}
\def\ellpp{{\ell^{\prime \prime}}}
\def\ellppi{{\ell_i^{\prime \prime}}}
\def\ms{{M_z^\ast}}
\def\cl{{\rm cl}}


%Bbb
\def\C{\mathbb C}
\def\R{\mathbb R}
\def\T{\mathbb T}
\def\D{\mathbb D}
\def\B{\mathbb B}
\def\Z{\mathbb Z}
\def\NN{\mathbb N}
\def\bm{{\mathbb B}_m}
\def\KK{{\mathbf K}}
\def\LLL{{\mathbf L}}

%Modified symbols
\def\inn{\ \in \ }

%Commands
\def\dis{\displaystyle}

%Set-up
\def\be{\setcounter{equation}{\value{theorem}} \begin{equation}}
\def\ee{\end{equation} \addtocounter{theorem}{1}}
\def\beq{\begin{eqnarray*}}
\def\eeq{\end{eqnarray*}}
\def\se{\setcounter{equation}{\value{theorem}}} 
\def\att{\addtocounter{theorem}{1}}
\def\vs{\vskip 5pt}
\def\bs{\vskip 12pt}
\def\exer{\bs \att {{\bf Exercise \thetheorem \ }} }
\def\exam{\bs \att {{\bf Example \thetheorem \ }} }
\def\prob{\bs \att {{\bf Problem \thetheorem \ }} }
\def\quest{\bs \att {{\bf Question \thetheorem \ }} }
%\def\rem{\bs \att {{\bf Remark \thetheorem \ }} }
\def\bp{{\sc Proof: }}
\def\ep{{}{\hfill $\Box$} \vskip 5pt \par}
\def\endpfeq#1{\newline{\mbox{}\hfill$\displaystyle#1$\hfill\Box}}
\def\endpfarray{\vskip - 4 ex \rightline{\tombstone}\medskip}
%\def\bp{\begin{proof}}
%\def\ep{\end{proof}}
\def\oep{{\hspace*{\fill} $\Box$} \vskip 5pt \par}
\def\obc{{\sc Proof of Claim: }}
\def\oec{{}{\hspace*{\fill} $\lhd$} \vskip 5pt \par}
\def\bl{\begin{lemma}}
\def\el{\end{lemma}}
\def\bt{\begin{theorem}}
\def\et{\end{theorem}}
\def\bprop{\begin{prop}}
\def\eprop{\end{prop}}
\def\bd{\begin{definition}}
\def\ed{\end{definition}}
\def\br{\begin{remark}}
\def\er{\end{remark}}
\def\bexer{\begin{exercise}}
\def\eexer{\end{exercise}}
\def\bfig{\begin{figure}}
\def\efig{\end{figure}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{schol}[theorem]{Scholium}
\newtheorem{porism}[theorem]{Porism}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{defin}[theorem]{Definition}

\newtheorem{claim}[theorem]{Claim}

\newtheorem{othm}{Theorem}

%\theoremstyle{definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{definition}[theorem]{Definition}


\renewcommand{\theequation}{\thesection.\arabic{equation}}    


